Impossibility of composable Oblivious Transfer in relativistic quantum cryptography

We study the cryptographic primitive Oblivious Transfer; a composable construction of this resource would allow arbitrary multi-party computation to be carried out in a secure way, i.e. to compute functions in a distributed way while keeping inputs from different parties private. First we review a framework that allows us to analyze composability of classical and quantum cryptographic protocols in special relativity: Abstract Cryptography implemented with Causal Boxes. We then (1) explore and formalize different versions of oblivious transfer found in the literature, (2) prove that their equivalence holds also in relativistic quantum settings, (3) show that it is impossible to composably construct any of these versions of oblivious transfer from only classical or quantum communication among distrusting agents in relativistic settings, (4) prove that the impossibility also extends to multi-party computation, and (5) provide a mutual construction between oblivious transfer and bit commitment.

==> figure/coin-flip.tex <==
\begin{tikzpicture}[scale=1.5]
    \acresource{$CF$}{0}{0}{1}{1}
    \acleftmessage[<-]{$(x, P_A)$}{0.5}{-0.75}{0}
    \acrightmessage[->]{$(x, P_B)$}{0.5}{1}{1.75}
\end{tikzpicture}
